Super-massive planets around late-type stars - the case of OGLE-2012-BLG-0406Lb

The core accretion theory of planetary formation does not predict that super-Jupiters will form beyond the snow line of a low mass stars. We present a discovery of 3.9 +- 1.2 M_Jup mass planet orbiting the 0.59 +- 0.17 M_Sun star using the gravitational microlensing method. During the event, the projected separation of the planet and the star is 3.9 +- 1.0 AU i.e., the planet is significantly further from the host star than the snow line. This is a fourth such planet discovered using the microlensing technique and challenges the core accretion theory.

==> tab_res.tex <==
$\chi^2$ &    &  $1651.96$ &   &  $1665.56$ &  $1676.42$ &  $1701.95$ &  $1712.83$ \\
 ${\rm dof}$  &  &  $1652$  &  &  $1652$  &  $1650$  &  $1650$  &  $1648$   \\
$\frac{f_b}{f_s}$  &    &  $0.039$ &  $0.035$ &  $0.006$ &  $-0.028$ &  $-0.072$ &  $-0.069$ \\
 &  &  $\pm0.021$  &  $\pm0.019$  &  $\pm0.020$  &  $\pm0.020$  &  $\pm0.006$  &  $\pm0.006$   \\
$t_0-6141$  &  d   &  $0.548$ &  $0.576$ &  $0.583$ &  $0.676$ &  $0.736$ &  $0.593$ \\
 &  &  $\pm0.090$  &  $\pm0.077$  &  $\pm0.093$  &  $\pm0.075$  &  $\pm0.048$  &  $\pm0.031$   \\
$u_0$  &  $r_{\rm E}$   &  $0.5065$ &  $0.5080$ &  $-0.5169$ &  $0.5257$ &  $0.5441$ &  $0.5425$ \\
 &  &  $\pm0.0068$  &  $\pm0.0060$  &  $\pm0.0065$  &  $\pm0.0068$  &  $\pm0.0024$  &  $\pm0.0022$   \\
$t_{\rm E}$  &  d  &  $64.33$ &  $64.23$ &  $61.94$ &  $63.79$ &  $62.25$ &  $62.63$ \\
 &  &  $\pm0.49$  &  $\pm0.44$  &  $\pm0.81$  &  $\pm0.54$  &  $\pm0.27$  &  $\pm0.16$   \\
$\pi_{{\rm E}, N}$  &    &  $-0.118$ &  $-0.117$ &  $0.232$ &  -  &  $-0.026$ &  -  \\
 &  &  $\pm0.026$  &  $\pm0.026$  &  $\pm0.078$  &  &  $\pm0.021$  &   \\
$\pi_{{\rm E}, E}$  &    &  $0.046$ &  $0.046$ &  $0.020$ &  -  &  $0.029$ &  -  \\
 &  &  $\pm0.010$  &  $\pm0.010$  &  $\pm0.008$  &  &  $\pm0.010$  &   \\
$\rho$  &    &  $0.0109$ &  $0.0103$ &  $0.0093$ &  $0.0074$ &  $0.0097$ &  $0.0098$ \\
 &  &  $\pm0.0013$  &  $\pm0.0009$  &  $\pm0.0013$  &  $\pm0.0014$  &  $\pm0.0004$  &  $\pm0.0004$   \\
$q$  &  $10^{-3}$  &  $6.26$ &  $5.85$ &  $5.40$ &  $4.17$ &  $5.85$ &  $5.78$ \\
 &  &  $\pm0.78$  &  $\pm0.46$  &  $\pm0.64$  &  $\pm0.53$  &  $\pm0.10$  &  $\pm0.08$   \\
$s_0$  &  $r_{\rm E}$   &  $1.3134$ &  $1.3174$ &  $1.3289$ &  $1.3453$ &  $1.3514$ &  $1.3500$ \\
 &  &  $\pm0.0091$  &  $\pm0.0063$  &  $\pm0.0085$  &  $\pm0.0087$  &  $\pm0.0017$  &  $\pm0.0016$   \\
$\alpha_0$  &  deg    &  $47.98$ &  $48.04$ &  $-47.40$ &  $49.29$ &  $49.35$ &  $49.58$ \\
 &  &  $\pm0.29$  &  $\pm0.26$  &  $\pm0.60$  &  $\pm0.18$  &  $\pm0.14$  &  $\pm0.09$   \\
$\gamma_\parallel$  &  ${\rm yr}^{-1}$  &  $-0.46$ &  $-0.39$ &  $-0.22$ &  $0.06$ &  -  &  -  \\
 &  &  $\pm0.16$  &  $\pm0.10$  &  $\pm0.15$  &  $\pm0.15$  &  &   \\
$\gamma_\perp$  &  ${\rm rad}~{\rm yr}^{-1}$  &  $0.57$ &  $0.31$ &  $0.29$ &  $-0.90$ &  -  &  -  \\
 &  &  $\pm0.51$  &  $\pm0.31$  &  $\pm0.48$  &  $\pm0.44$  &  &   \\

